A Compositional Algorithm for the Conflict-Free Electric Vehicle Routing Problem

The Conflict-Free Electric Vehicle Routing Problem (CF-EVRP) is an extension of the Vehicle Routing Problem (VRP), a combinatorial optimization problem of designing routes for vehicles to visit customers such that a cost function, typically the number of vehicles or the total travelled distance, is minimized. The problem finds many logistics applications, particularly for highly automated logistic systems for material handling. The CF-EVRP involves constraints such as time windows on the delivery to the customers, limited operating range of the vehicles, and limited capacity on the number of vehicles that a road segment can accommodate at the same time. In this paper, the compositional algorithm ComSat for solving the CF-EVRP is presented. The algorithm iterates through the sub-problems until a globally feasible solution is found. The proposed algorithm is implemented using an optimizing SMT-solver and is evaluated against an implementation of a previously presented monolithic model. The soundness and completeness of the algorithm are proven, and it is benchmarked on a set of generated problems and found to be able to solve problems of industrial size.

==> MF_OnOptimality.tex <==
h\section*{Appendix: Ideas on the optimality of ComSat}

Here are my thoughts on how we could prove that ComSat actually computes the true optimum. Unfortunately, I think this reasoning now shows that we are not guaranteed this.

ComSat first computes \emph{path assignments}, $P_i$. There is a finite number of these (prove this!), and they can be ordered according to some cost function such that: 
$$ P'_1\leq P'_2\leq\dots\leq P'_n.$$
($P'_i$ denotes the cost function value of $P_i$.)

Two things:
\begin{enumerate}
    \item ComSat computes the path assignments in ascending order of cost function value; this needs to be proven.
    \item There can exist two path assignments, $P_i$ and $P_{i+1}$ such that $P'_i=P'_{i+1}$; this is obvious.
\end{enumerate}

Now, for each path assignment $P_i$, there exists a finite (prove this!) set of \emph{route assignments}, $R_{i,j}$, that can be ordered according to some cost function such that:
$$R'_{i,1}\leq R'_{i,2}\leq\dots\leq R'_{i,m}.$$
(Again, $R'_{i,j}$ denotes the cost function value of $R_{i,j}$.)

%%MF Two things also here, but only the first one is really important:
One important thing here:
\begin{enumerate}
    \item ComSat computes for each path assignment the corresponding route assignments in ascending order; this needs to be proven.
%%MF    \item If a route assignment is ``too much'' infeasible, ComSat does not check the rest of the route assignments, but goes straight for the next path assignment; this is just an optimization of the algorithm.
\end{enumerate}

ComSat now checks if the route assignments are feasible, and it does this respecting the orderings defined above. If none of the route assignments for a certain path assignment $P_i$ are feasible, the route assignments for $P_{i+1}$ are checked (again, in order). That this really is the case needs to be shown, but assuming now that this is the actual behavior, how can we use this knowledge to show that ComSat indeed computes the true optimum?

\textbf{Claim:} If it can be proven that for two path assignments $P_i$ and $P_{i+1}$ with $P'_i\leq P'_{i+1}$, the worst route assignment for $P_i$ is better than the best route assignment for $P_{i+1}$, that is that 
\begin{equation}\label{eq:wellBehaved}
    R'_{i,m}\leq R'_{i+1,1}
\end{equation}
then (it should be possible to prove that) ComSat always returns the true optimum.

And the reasoning would go like this: Once ComSat has found a feasible route assignment, if~\eqref{eq:wellBehaved} holds and ComSat explores the path and route assignments in ascending order, from better to worse, we know that no route assignment, and hence no path assignment, with better cost is feasible. 
%%MF This builds on~\eqref{eq:wellBehaved} and that ComSat explores the path and route assignments in ascending order, from better to worse.

\subsection*{However\dots}

Since there can exist two path assignments, $P_i$ and $P_{i+1}$ such that $P'_i=P'_{i+1}$, their order is not well-defined, and so~\eqref{eq:wellBehaved} is not guaranteed. It could very well be that the opposite to~\eqref{eq:wellBehaved} holds and we have no way of knowing this when selecting which of $P_i$ or $P_{i+1}$ to compute route assignments for first. Therefore, we could pick a feasible route assignment with a worse value than a feasible route assignment corresponding to the other path assignment.



==> MF_thoughts.tex <==
As I have already mentioned, I am reviewing v2 of a paper on 3D bin packing by Mariagrazia and co-authors. One thing they do there is to solve the global problem, they solve to optimality two sub-problems, and then use a heuristic to from those solutions put together a solution to the global problem.; they say " the proposed method is based on a combination of the exact solution of two mathematical models and a heuristic approach". The common term for this appears to be "matheuristic"; teh paper refers to this paper https://link.springer.com/content/pdf/10.1007%2F978-3-319-07153-4_14-1.pdf by Fischetti and Fischetti, but there's also a wikipedia page on it https://en.wikipedia.org/wiki/Matheuristics.

To me, this sounds (on a high abstraction level) similar to what CompSAT does. So... maybe the word "matheuristic" should be used?

Waddayathunk?

#######################################

I have been reviewing a paper that has Mariagrazia Dotoli as co-author. The paper was originally titled "Automating Bin Packing: a Layer Building Optimization Module for Cost Effective Logistics" but is now on its second round renamed to "Automating Bin Packing: a Layer Building Matheuristics for Cost Effective Logistics". But the reason for this email is to quote the authors' summary of their changes for the second version:

Summary of the main changes
We thank the Associate Editor and the Reviewers for their helpful and constructive comments and suggestions,
which guided us towards a revision of the paper, summarized as follows:
1. We rephrased and better organized the Abstract, Introduction, and State of the Art (Sections I and II) to present
the related contents in a more concise and significant way.
2. We enriched the discussion of the state of the art (Section II) by including additional meaningful references.
3. We reformulated the three-dimensional single bin size bin packing problem (3D-SBSBPP) mathematical models
in Sections IV and Appendix A.
4. We renamed the proposed approach (and consequently the title of the paper) as a matheuristics to suitably
identify the underlying features based both on exact method and heuristics.
5. We improved the Experimental Results section (Section VI) by providing: (1) a more detailed comparison of
the results obtained by the proposed algorithm and by the exact method for the 3D-SBSBPP; (2) a comparison
of the proposed algorithm with a literature bin packing matheuristics considering a higher number of instances;
(3) a more detailed performance analysis of the proposed algorithm on the real industrial data-set.
6. We checked the whole paper for typos and unclear sentences.
In the sequel we detail the changes made to the article in response to the Associate Editor and the Reviewers.
Please, note that all changes are highlighted in blue font in the revised manuscript.

This may give some insights for us as to how to update our own paper. Note especially point 5, above.

And one other thing, they put all new text in blue, I think this is a good thing to do, to make it show up clearly.



==> NtP_orig.tex <==
%%MF The original NtP (Oct 30, 2021)
    The need to define and efficiently solve the  \theModel relates to an industrial application where a fleet of autonomous moving robots navigate in a heterogeneous environment, where humans and other vehicles share the work space with the robots. Such a scenario requires the robots to be able to react to external events to guarantee both the safety of the surrounding resources and the accomplishment of the jobs they are assigned to. 
    Implementing a distributed system where each robot has the ability to compute an optimal plan to execute its job would require highly advanced robots and may be very expensive for large fleets. On the other hand, centralizing the computation of the robots' paths would allow to use less sophisticated robots equipped with only basic sensors to avoid immediate danger. 
    
    To compute a schedule for a fleet of robots is a hard task, since several aspects must simultaneously be taken into account. 
    % First and foremost, deadlines on the deliveries must be met, in order to avoid disruptions in the manufacturing/assembly line; at the same time, earliest arrival time are needed to avoid queues at the workstations. Also, as robots have limited operating range, their schedule must account for charging times, when robots are not available. Moreover, there exist task-specific requirements on the types of robots, as well as order of execution of tasks. Last but not least, the schedule must take into account the road segments capacity in terms of vehicles that can be accommodated simultaneously. This means that if too many vehicles take the same path they could block each other's way. 
    One approach is to break down the overall scheduling problem into sub-problems that are easy to solve, and then incrementally build a schedule based on the solutions of the sub-problems.
    The compositional algorithm (\theAlgorithm) we present in this work is based on this idea and can provide feasible schedules for fleets of robots within minutes. 
    For particularly hard problems of the \theModel, \theAlgorithm could take a long time to compute a schedule due to all the possible solutions to explore. 
    However, in real industrial scenarios there is usually a reasonable number of robots available compared to the number of jobs to execute and the plant layout is not excessively complicated. In such scenarios, \theAlgorithm shows considerable performance.

==> SR_state_space_analysis.tex <==


%%MF Before going into the algorithm's details, it is worth analyzing where the main complexity of the problem lies. 
%%MF As mentioned above, to deal with capacity constraints it is necessary to keep track of the vehicles' location at each point in time, consequently, time discretization is needed. 
%%MF As noted above, time is discretized to be able to keep track of each vehicle's location at each point in time.
By analyzing the state space\MFedit{complexity}{} of the problem, with and without considering capacity constraints, it can be determined how the problem parameters affect the problem size.
Although the state space growth is not directly proportional to the solving time, it provides an idea of the complexity of the problem itself.
For instance, a monolithic model for the example above (where capacity constraints are considered), would be so large that even the model generation time would be non-negligible, if at all possible, due to memory limitation.
In order to be able to compute the state space size, the domains of the real variables are restricted to integers.  

The parameters needed to analyze the state space  are the number of tasks $|\taskSet|$, the number of nodes $|\nodeSet|$ in the graph representing  the plant, the number of vehicles $|\vehicleSet|$, the time horizon \timeHorizon, and the operating range of the vehicles \OR.

In the case capacity constraints are not considered, based on the model formulation from \cite{schneider2014electric}, 
% the decision variables needed are:
% \begin{itemize}[label={},leftmargin=*]
%     \item $\tau_{ik}$: integer decision variable modelling the arrival time of vehicle $i \in \vehicleSet$ at customer $k \in \taskSet$. The domain of this variables spans from $0$ to \timeHorizon.
%     \item $rc_{ik}$: integer decision variable modelling the remaining charge of vehicle $i \in \vehicleSet$ when arriving at customer $k \in \taskSet$. The domain of this variables spans from $0$ to \OR.
%     \item $x_{ik_1k_2}$: Boolean decision variable modelling direct travel from task $i \in \vehicleSet$ to task $j_1,j_2 \in \taskSet$.
% \end{itemize}
% For such a set of variables and parameters,
the state space complexity, including both legal and illegal states is 
$$\OR^{|\vehicleSet|\cdot|\taskSet|}\cdot \timeHorizon^{|\vehicleSet|\cdot|\taskSet|}\cdot 2^{|\vehicleSet|\cdot 2|\taskSet|}$$
which can be rewritten as 
$$ 2^{|\vehicleSet|\cdot |\taskSet| \cdot (\log_2{(\OR\cdot\timeHorizon)} + 2))} $$

If capacity constraints are considered, based on the model formulation from \cite{roselli2021smt},
% the decision variables needed are:
% \begin{itemize}[label={},leftmargin=*]
%     \item $x_{ik}$: Boolean decision variable modelling the assignment of vehicle $i \in \vehicleSet$ to task $k \in \taskSet$.
%     \item $z_{ikt}$: Boolean decision variable modelling the service of vehicle $i \in \vehicleSet$ to task $k \in \taskSet$ at time $t \in \{0,\ldots,\timeHorizon \}$.
%     \item $rc_{it}$: integer decision variable modelling the remaining charge of vehicle $i \in \vehicleSet$ at time $t \in \{0,\ldots,\timeHorizon \}$. The domain of this variables spans from $0$ to \OR.
%     \item $at_{int}$: Boolean decision variable that is true if vehicle $i \in \vehicleSet$ is at node $n \in \nodeSet$ at time $t \in \{0,\ldots,\timeHorizon \}$.
%     \item $move_{int}$: Boolean decision variable that is true if vehicle $i \in \vehicleSet$ at time $t \in \{0,\ldots,\timeHorizon \}$ decides to move to node node $n \in \nodeSet$.
% \end{itemize}
% For such a set of variables and parameters,
the state space complexity, including both legal and illegal states is

\begin{equation}\label{eq:statespace}
2^{|\vehicleSet|\cdot|\taskSet|} 
\times
2^{|\vehicleSet|\cdot|\taskSet|\cdot \timeHorizon}
\times
\OR^{|\vehicleSet|\cdot\timeHorizon}
\times 
2^{2\cdot|\vehicleSet|\cdot|\nodeSet|\cdot \timeHorizon}
\end{equation}
which can be rewritten as 
\begin{equation}\label{eq:statespacesize}
2^{|\vehicleSet| ( |\taskSet|+\timeHorizon (2|\nodeSet| + \log_2{(\OR)} + |\taskSet| )  )} 
\end{equation}

When capacity constraints are not considered, the number of vehicles $|\vehicleSet|$ and the number of tasks $|\taskSet|$ directly affect the exponential growth of the state space, while the operating range \OR and the time horizon $\timeHorizon$ contribution is diminished since they appear in the exponent as a binary logarithm.  

On the other hand, when capacity constraints are considered, due to time discretization, a larger set of variables is required to model the system. In this case, the time horizon \timeHorizon, the number of vehicles $|\vehicleSet|$, the number of tasks $|\taskSet|$ and the number of nodes $|\nodeSet|$ directly affect the exponential growth of the state space.

For instance, in the example above, the exponent's value in case capacity constraints are not considered would be \emph{609}, while in case capacity constraints are considered, the exponent's value would be $\approx 112\,185$.
 

Moreover, when discretizing time, it is not possible to deal with problems where non-integer parameters are involved. From these conclusions it is evident that time discretization must be avoided, hence the need to break down the problem in order to achieve such goal. 

==> relevant_corner_cases.tex <==
\section{Relevant Corner Cases}
 In order to discuss the above assumptions and the following restrictions, we introduce some relevant corner cases that may occur in an instance of the \theModel.
 
\subsection{Solution requires cycles in the walks} \label{counterex:no_cycles}
Figure~\ref{fig:no_cycles} shows an example of how walks containing cycles may be required to solve an instance of the \theModel. In this example all edges have length (normal font) and capacity (subscript) equal to \emph{1}; vehicles \emph{R1} and \emph{R2} are initially located at nodes \emph{1} and \emph{2}, respectively, both having operating range equal to \emph{5}, while tasks \emph{T1} and \emph{T2} are located at nodes \emph{3} and \emph{1}; Task \emph{T1} needs Vehicle \emph{R1} to visit Node \emph{3} within time-step \emph{0} and \emph{5}, while Task \emph{T2} needs Vehicle \emph{R2} to visit Node \emph{1} also within time-step \emph{0} and \emph{5}. For \emph{R1} to be able to leave Node \emph{1}, \emph{R2} has to move to \emph{4}. Afterwards it goes back to Node \emph{2} before moving to Node \emph{1}, thus describing a cycle (it visits one node more than once).

\begin{figure}[h]
    \centering
    \includegraphics[width = 0.34\textwidth]{pics/counter_example_no_cyclic_paths.pdf}
    \caption{Counter example to show need for cycles in the walks.}
    \label{fig:no_cycles}
\end{figure}

We restrict the problem to forbid cycles in the walks and we are going to use this assumption in Section~\ref{sec: proofs} to prove completeness; however, we are going to show that even when cycles are allowed, completeness can be guaranteed. 

\subsection{Solution requires different paths for different routes that involve the same two customers}
Figure~\ref{fig:same_path_diff_routes} shows an example of why different routes may need different paths if such paths share the start and end node. In fact, different tasks may be located at the same node, so it is possible that two vehicles need to start or end at the same location. However, due to problem requirements such as time windows, a feasible schedule may only be achieved by having the vehicles use different paths. Let us assume that nodes \emph{1} and \emph{2} are hubs and each edge has capacity and length equal to \emph{one}, except for Edge \emph{(1,2)}, whose length is 2. Both tasks \emph{T1} and \emph{T2} are located at Node \emph{2}, require vehicles \emph{R1} and \emph{R2} respectively, and need to be served before time-step \emph{2}. The only way the vehicles can meet the time windows is if they take different paths to travel from Node \emph{1} to node \emph{2},

\begin{figure}[h]
    \centering
    \includegraphics[width = 0.24\textwidth]{pics/counter_example_same_paths_different_routes.pdf}
    \caption{Counter example illustrating the need for different paths in different routes.}
    \label{fig:same_path_diff_routes}
\end{figure}

We initially compute paths to travel from any customer to any other customer and those paths are used to design the routes that vehicles will be assigned to in order to serve the customers; to this point all routes will use the same path to travel from one node to another. Hence the problem will be initially declared unfeasible.
However, the algorithm will try to change the paths, and in doing so, it will specify which route the path is for, so that different routes can have different paths to travel from and/or to the same location.

\subsection{Intrinsic unfeasibility}

Figure~\ref{fig:intrinsic_unfeasibility} shows an example of a problem instance that is unfeasible due to the lack of available vehicles to execute the jobs. While in some cases it could be possible to immediately determine whether an instance is feasible or not, some other cases involve more subtle reasoning. In the example, vehicle \emph{R1}, whose operating range is \emph{2} distance units is located at Node \emph{1}, while tasks \emph{T1} and \emph{T2} are located at nodes \emph{2} and \emph{3} respectively, they both must be served before time-step \emph{2} and they both require vehicle \emph{R1}. The problem is unfeasible because the vehicle need to recharge after executing one task but the time windows are too strict to allow it.

\begin{figure}[h]
    \centering
    \includegraphics[width = 0.24\textwidth]{pics/counter_example_intrinsic_unfeasibility.pdf}
    \caption{Counter example illustrating intrinsic unfeasibility of an instance.}
    \label{fig:intrinsic_unfeasibility}
\end{figure}

The algorithm can design routes to serve the customers, but it will fail to assign vehicles to them. It will then try different routes and try to assign vehicles again, until no routing is possible any longer. For larger problems the number of possible combinations of routes can be significantly large, and the algorithm will have to try them all before declaring an instance unfeasible. 

==> some_notes_on_completeness.tex <==
If capacity constraints are not included, it means that I do not need to worry about vehicles being at the same node or edge at the same time. Hence there is no need to look for alternative paths, all I need is one path between any two customers and I'll use the shortest because they guarantee the shortest travelling distance and, therefore, the short travelling time. 

WHAT A SOLUTION LOOKS LIKE:
\begin{itemize}
    \item a set of routes such that each customer is served within its time window
    \item a match between each route and one of the available vehicles such that constraints on the operating range and charging rate are met.
\end{itemize}

I assume that the algorithms that Z3 uses are sound and complete. 
I know there is a finite number of solutions to the routing problem. This can be proved using graph theory because routes are cycles in graphs and their number is finite. In our case there are even fewer solutions because of the time windows.

using Z3 I can enumerate them all. For each solution, I can use Z3 to check whether there exist an assignment of vehicles. 

IF A SOLUTION DOES NOT EXISTS:

\begin{itemize}
    \item either there is no set of routes that satisfies the constraints on the time windows
    \item or the vehicles I have are not enough (in number and/or type) to execute them
\end{itemize}

also in this case I will get the right solution because I am checking every possible solution to the \emph{routing problem} and then checking if it satisfies the \emph{assignment problem}; Figure~\ref{fig:relaxed_problem} shows this graphically. 

To sum up, if I relax the capacity constraint I am left with an optimization problem (the \emph{routing problem}) and a feasibility check with respect to the available vehicles (\emph{assignment problem}). Assuming Z3 algorithms are complete, my algorithm will be complete too.

In this case I need to make sure that my solution is conflict free. This means that the shortest paths are not necessarily the best ones because I may need to take detours to avoid other vehicles. However as long as the number of paths is finite, I can still guarantee completeness. 

\textcolor{green}{I don't know if the following needs formal proof or we can just state it:} I assume that, given a weighed, directed graph, there is a finite number of \emph{walks} of a fixed length \emph{l}. Such length \emph{l} can be calculated based on the time windows.

IF A SOLUTION EXISTS, IT WILL LOOK LIKE THIS
\begin{itemize}
    \item a set of routes such that each customer is served within its time window
    \item a vehicle assigned to each route such that the vehicle has always a non-negative charge (it is a different phrasing of what I stated in the previous subsection, but the meaning is the same...I don't know which one is better)
    \item there is never more vehicles at a node (edge) than allowed (no-swap is allowed either)
\end{itemize}

\emph{Definition 1}:To be more specific, a solution is a set of routes where, for each route, it is specified the arrival time at each node included in the route.

The algorithm first finds a feasible routing based on the shortest path between any two customers. Then it checks if there are vehicles to execute the current routes. Under the assumption that all vehicles have the same operating range all assignments are equivalent, hence if the following step is \emph{unsat} there is no need to try a different one (they will also be \emph{unsat}). 

If there is a feasible assignment but the \emph{Scheduling Problem} is \emph{unsat} the algorithm will iteratively replace the paths until the \emph{Scheduling Problem} is \emph{sat} or until all combinations of paths have been tried. If all paths are tried unsuccessfully the algorithm will backtrack to the \emph{Routing Problem} and find another sets of routes. 

\textcolor{red}{I think the following paragraph is the key to prove completeness}

Since the algorithm checks all possible set of routes, it will eventually hit one of the \emph{feasible} ones. Moreover, since it tries all possible combinations of paths, and different paths lead to different arrival times at the nodes included in a route, it will eventually find the feasible arrival time for each node of each route


IF A SOLUTION DOES NOT EXIST

The algorithm will check all possible sets of routes, and for each set, it will check all possible combinations of paths, before declaring the problem \emph{unsat} 

SOME REMARKS ABOUT THE IMPLEMENTATION

\textcolor{red}{this part will probably be spread in the subsections where I introduce the sub-problems, but it is good to write it down for now. } The algorithm may be quite inefficient if the the solution is hard to find due to the capacity constraint, because the number of possible \emph{walks} can be tremendously large. Therefore in practice it would be convenient to change routes after we have checked a certain number of combinations of paths. This, in combination with some cost function that prioritize paths that do not overlap a lot (I am just brainstorming here) could be quite effective. We could also try to figure out (if they exist) some conditions that will shrink the set of feasible paths.

==> tables/table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{Evaluation of the compositional algorithm for the \theModel ~over a set of generated problem instances. Instances are sorted by the parameters N-V-J (nodes, vehicles, jobs), and value of edge reduction in the columns, and time horizon in the rows. For each resulting class, five instances are evaluated and the number of satisfied (sat), unsatisfied (unsat), and unknown ones is reported, together with the average solving time (in seconds). The symbol ``-'' means that no instance for that category was either satisfiable or unsatisfiable or unknown, depending on where the symbol appears.}
            \begin{tabular}{cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
    \toprule
       &    & \multicolumn{6}{c|}{15-3-5} & \multicolumn{6}{c|}{25-4-7} & \multicolumn{6}{c|}{35-6-8} & \multicolumn{6}{c}{35-6-10} \\
    T  &    & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{25} & \multicolumn{2}{c|}{50} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{25} & \multicolumn{2}{c|}{50} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{25} & \multicolumn{2}{c|}{50} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{25} & \multicolumn{2}{c}{50} \\
    \midrule
       & sat & 4  & 2  & 4  & 2  & 2  & 2  & 3  & 8  & 3  & 41 & 3  & 26 & 0  & -  & 0  & -  & 0  & -  & 2  & 56 & 0  & -  & 0  & - \\
    30 & unsat & 1  & 0  & 1  & 0  & 2  & 0  & 0  & -  & 0  & -  & 0  & -  & 1  & 1  & 2  & 21 & 3  & 1  & 0  & -  & 1  & 1  & 1  & 1 \\
       & unknown & 0  & -  & 0  & -  & 1  & 11 & 2  & 27 & 2  & 23 & 2  & 21 & 4  & 133 & 3  & 130 & 2  & 107 & 3  & 36 & 4  & 40 & 4  & 35 \\
    \midrule
       & sat & 4  & 2  & 4  & 2  & 3  & 3  & 3  & 14 & 4  & 15 & 2  & 7  & 0  & -  & 0  & -  & 0  & -  & 2  & 29 & 0  & -  & 1  & 46 \\
    40 & unsat & 1  & 0  & 1  & 0  & 2  & 0  & 0  & -  & 0  & -  & 0  & -  & 1  & 1  & 2  & 25 & 3  & 1  & 0  & -  & 1  & 0  & 1  & 0 \\
       & unknown & 0  & -  & 0  & -  & 0  & -  & 2  & 31 & 1  & 30 & 3  & 30 & 4  & 175 & 3  & 170 & 2  & 139 & 3  & 45 & 4  & 51 & 3  & 39 \\
    \midrule
       & sat & 4  & 2  & 4  & 3  & 3  & 3  & 4  & 25 & 4  & 9  & 3  & 9  & 1  & 169 & 1  & 242 & 0  & -  & 2  & 7  & 1  & 6  & 2  & 6 \\
    50 & unsat & 1  & 0  & 1  & 0  & 2  & 0  & 0  & -  & 0  & -  & 0  & -  & 1  & 1  & 2  & 29 & 3  & 1  & 0  & -  & 1  & 1  & 1  & 1 \\
       & unknown & 0  & -  & 0  & -  & 0  & -  & 1  & 44 & 1  & 38 & 2  & 40 & 3  & 226 & 2  & 173 & 2  & 172 & 3  & 83 & 3  & 76 & 2  & 59 \\
    \midrule
       & sat & 4  & 2  & 4  & 1  & 3  & 3  & 4  & 11 & 4  & 34 & 3  & 19 & 2  & 117 & 2  & 147 & 0  & -  & 3  & 11 & 1  & 2  & 1  & 2 \\
    60 & unsat & 1  & 0  & 1  & 0  & 2  & 0  & 0  & -  & 0  & -  & 0  & -  & 1  & 1  & 2  & 35 & 3  & 1  & 0  & -  & 1  & 1  & 1  & 1 \\
       & unknown & 0  & -  & 0  & -  & 0  & -  & 1  & 52 & 1  & 45 & 2  & 47 & 2  & 237 & 1  & 170 & 2  & 202 & 2  & 79 & 3  & 90 & 3  & 72 \\
    \bottomrule
    \end{tabular}%
  \label{tab:table_1}%
\end{table*}%


==> tables/test_table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{sidewaystable}[htbp]
  \centering
  \caption{Evaluation of ComSat for the \theModel ~over a set of generated problem instances. Instances are sorted by the parameters N-V-J (nodes, vehicles, jobs), and value of edge reduction in the columns, and time horizon in the rows. For each resulting class, five instances are evaluated and the number of feasible and unfeasible problems is reported, together with the average solving time (in seconds). The symbol ``- means that no instance for that category was either feasible or unfeasible, depending on where the symbol appears.}
  
     \resizebox{\columnwidth}{!}{%

  
    \begin{tabular}{c|cccccccccccccccccccccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{3}[4]{*}{}} & \multicolumn{24}{c}{N-V-J} \\
\cmidrule{2-25}    \multicolumn{1}{c}{} & \multicolumn{12}{c}{35-6-8 }                              & \multicolumn{12}{c}{35-07-10} \\
    \multicolumn{1}{c}{} & \multicolumn{12}{c}{Edge Reduction}                       & \multicolumn{12}{c}{Edge Reduction} \\
    \midrule
    T  & \multicolumn{4}{c}{0} & \multicolumn{4}{c}{25} & \multicolumn{4}{c}{50} & \multicolumn{4}{c}{0} & \multicolumn{4}{c}{25} & \multicolumn{4}{c}{50} \\
       & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas \\
    40 & 98.32 & '3/5 & 292.11 & '2/5 & 42.93 & '2/5 & 383.28 & '3/5 & 10.86 & '2/5 & 351.63 & '3/5 & 5.49 & '1/5 & 1.33 & '2/5 & 0  & '0/5 & 1.33 & '2/5 & 0  & '0/5 & 403.6 & '3/5 \\
    70 & 79.55 & '3/5 & 269.74 & '2/5 & 19.89 & '2/5 & 0.86 & '3/5 & 42.98 & '2/5 & 0.86 & '3/5 & 238.65 & '3/5 & 1.32 & '2/5 & 127.31 & '1/5 & 1.33 & '2/5 & 4.59 & '1/5 & 1.31 & '2/5 \\
    100 & 15.35 & '3/5 & 89.12 & '2/5 & 79.9 & '2/5 & 281.04 & '3/5 & 73.86 & '2/5 & 281.66 & '3/5 & 452.1 & '3/5 & 1.31 & '2/5 & 22.01 & '1/5 & 1.33 & '2/5 & 7.48 & '1/5 & 1.31 & '2/5 \\
    150 & 8.94 & '3/5 & 100.53 & '2/5 & 47.33 & '3/5 & 0.87 & '2/5 & 56.84 & '2/5 & 0.86 & '3/5 & 28.44 & '3/5 & 1.3 & '2/5 & 16.79 & '1/5 & 1.39 & '2/5 & 32.41 & '1/5 & 1.31 & '2/5 \\
    200 &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &  \\
    300 &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &  \\
    \midrule
    \multicolumn{1}{c}{\multirow{3}[4]{*}{}} & \multicolumn{24}{c}{N-V-J} \\
\cmidrule{2-25}    \multicolumn{1}{c}{} & \multicolumn{12}{c}{35-6-8 }                              & \multicolumn{12}{c}{35-07-10} \\
    \multicolumn{1}{c}{} & \multicolumn{12}{c}{Edge Reduction}                       & \multicolumn{12}{c}{Edge Reduction} \\
    \midrule
    T  & \multicolumn{4}{c}{0} & \multicolumn{4}{c}{25} & \multicolumn{4}{c}{50} & \multicolumn{4}{c}{0} & \multicolumn{4}{c}{25} & \multicolumn{4}{c}{50} \\
       & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas \\
    40 & 98.32 & '3/5 & 292.11 & '2/5 & 42.93 & '2/5 & 383.28 & '3/5 & 10.86 & '2/5 & 351.63 & '3/5 & 5.49 & '1/5 & 1.33 & '2/5 & 0  & '0/5 & 1.33 & '2/5 & 0  & '0/5 & 403.6 & '3/5 \\
    70 & 79.55 & '3/5 & 269.74 & '2/5 & 19.89 & '2/5 & 0.86 & '3/5 & 42.98 & '2/5 & 0.86 & '3/5 & 238.65 & '3/5 & 1.32 & '2/5 & 127.31 & '1/5 & 1.33 & '2/5 & 4.59 & '1/5 & 1.31 & '2/5 \\
    100 & 15.35 & '3/5 & 89.12 & '2/5 & 79.9 & '2/5 & 281.04 & '3/5 & 73.86 & '2/5 & 281.66 & '3/5 & 452.1 & '3/5 & 1.31 & '2/5 & 22.01 & '1/5 & 1.33 & '2/5 & 7.48 & '1/5 & 1.31 & '2/5 \\
    150 & 8.94 & '3/5 & 100.53 & '2/5 & 47.33 & '3/5 & 0.87 & '2/5 & 56.84 & '2/5 & 0.86 & '3/5 & 28.44 & '3/5 & 1.3 & '2/5 & 16.79 & '1/5 & 1.39 & '2/5 & 32.41 & '1/5 & 1.31 & '2/5 \\
    200 &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &  \\
    300 &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &    &  \\
\cmidrule{1-1}    \end{tabular}%
    
    }
    
  \label{tab:addlabel}%
\end{sidewaystable}%


==> tables/test_table_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{sidewaystable}[]
\begin{tabular}{ccccccccccccccccccccccccc}
\multirow{3}{*}{}    & \multicolumn{24}{l}{N-V-J}                                                                                                                                                                                                        \\
                     & \multicolumn{12}{l}{35-6-8}                                                                                     & \multicolumn{12}{l}{35-07-10}                                                                                   \\
                     & \multicolumn{12}{l}{Edge Reduction}                                                                             & \multicolumn{12}{l}{Edge Reduction}                                                                             \\
\multirow{5}{*}{T}   & \multicolumn{4}{l}{0}               & \multicolumn{4}{l}{25}              & \multicolumn{4}{l}{50}              & \multicolumn{4}{l}{0}               & \multicolumn{4}{l}{25}              & \multicolumn{4}{l}{50}              \\
                     & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas \\
                     & 98.32    & '3/5 & 292.11   & '2/5   & 42.93    & '2/5 & 383.28   & '3/5   & 10.86    & '2/5 & 351.63   & '3/5   & 5.49     & '1/5 & 1.33     & '2/5   & 0        & '0/5 & 1.33     & '2/5   & 0        & '0/5 & 403.6    & '3/5   \\
                     & 79.55    & '3/5 & 269.74   & '2/5   & 19.89    & '2/5 & 0.86     & '3/5   & 42.98    & '2/5 & 0.86     & '3/5   & 238.65   & '3/5 & 1.32     & '2/5   & 127.31   & '1/5 & 1.33     & '2/5   & 4.59     & '1/5 & 1.31     & '2/5   \\
                     & 15.35    & '3/5 & 89.12    & '2/5   & 79.9     & '2/5 & 281.04   & '3/5   & 73.86    & '2/5 & 281.66   & '3/5   & 452.1    & '3/5 & 1.31     & '2/5   & 22.01    & '1/5 & 1.33     & '2/5   & 7.48     & '1/5 & 1.31     & '2/5   \\
150                  & 8.94     & '3/5 & 100.53   & '2/5   & 47.33    & '3/5 & 0.87     & '2/5   & 56.84    & '2/5 & 0.86     & '3/5   & 28.44    & '3/5 & 1.3      & '2/5   & 16.79    & '1/5 & 1.39     & '2/5   & 32.41    & '1/5 & 1.31     & '2/5   \\
200                  & 6.48     & '4/5 & 0.86     & '1/5   & 23.19    & '2/5 & 351.15   & '3/5   & 102.8    & '2/5 & 350.46   & '3/5   & 202.68   & '3/5 & 1.32     & '2/5   & 66.64    & '1/5 & 1.34     & '2/5   & 21.18    & '1/5 & 1.29     & '2/5   \\
300                  & 8.99     & '4/5 & 0.88     & '1/5   & 34.1     & '3/5 & 0.86     & '2/5   & 17.21    & '2/5 & 0.86     & '3/5   & 74.12    & '3/5 & 1.34     & '2/5   & 6.36     & '1/5 & 1.33     & '2/5   & 79.27    & '1/5 & 1.35     & '2/5   \\
\multirow{3}{*}{}    & \multicolumn{24}{l}{N-V-J}                                                                                                                                                                                                        \\
                     & \multicolumn{12}{l}{35-9-12}                                                                                    & \multicolumn{12}{l}{35-11-15}                                                                                   \\
                     & \multicolumn{12}{l}{Edge Reduction}                                                                             & \multicolumn{12}{l}{Edge Reduction}                                                                             \\
T                    & \multicolumn{4}{l}{0}               & \multicolumn{4}{l}{25}              & \multicolumn{4}{l}{50}              & \multicolumn{4}{l}{0}               & \multicolumn{4}{l}{25}              & \multicolumn{4}{l}{50}              \\
                     & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas & Av.(sec) & Feas & Av.(sec) & Unfeas \\
40                   &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        \\
70                   &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        \\
\multirow{5}{*}{100} &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        \\
                     &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        \\
                     &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        \\
                     &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        \\
                     &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &        &          &      &          &       
\end{tabular}
\end{sidewaystable}
